Production Networks and War

How do severe shocks such as war alter the economy? We study how a country's production network is affected by a devastating but localized conflict. Using unique transaction-level data on Ukrainian railway shipments around the start of the 2014 Russia-Ukraine crisis, we uncover several novel indirect effects of conflict on firms. First, we document substantial propagation effects on interfirm trade--trade declines even between partners outside the conflict areas if one of them had traded with those areas before the conflict events. The magnitude of such second-degree effect of conflict is one-fifth of the first-degree effect. Ignoring this propagation would lead to an underestimate of the total impact of conflict on trade by about 67\%. Second, war induces sudden changes in the production-network structure that influence firm performance. Specifically, we find that firms that exogenously became more central--after the conflict practically cut off certain regions from the rest of Ukraine--received a relative boost to their revenues. Finally, in a production-network model, we separately estimate the effects of the exogenous firm removal and the subsequent endogenous network adjustment on firm revenue distribution. For a median firm, network adjustment compensates for 80\% of the network destruction a year after the conflict onset.

==> Tables/Table1_A.tex <==
%                    &       %est1        &       %est2        &       %est3        &       %est4        \\[-0.15cm]
Sending From $\times$ Post-August 2014&      -2.097$^{*}$  &      -7.636$^{***}$&      -1.558$^{***}$&      -1.427$^{**}$ \\[-0.15cm]
                    &     (1.059)        &     (0.881)        &     (0.487)        &     (0.595)        \\[-0.15cm]\addlinespace[0.15cm] 
Sending To $\times$ Post-August 2014&      -2.198$^{***}$&      -1.553$^{***}$&      -1.392$^{***}$&      -1.287$^{***}$\\[-0.15cm]
                    &     (0.529)        &     (0.404)        &     (0.320)        &     (0.202)        \\[-0.15cm]\addlinespace[0.15cm] 
Region From, Region To, Time FEs&{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        \\[-0.15cm]\addlinespace[0.15cm] 

R$^2$               &        0.30        &        0.37        &        0.36        &        0.43        \\[-0.15cm]
Observations        &    {97,040}        &    {97,040}        &    {97,040}        &    {97,040}        \\[-0.15cm]
\addlinespace[0.15cm] 


==> Tables/Table1_B.tex <==
%                    &       %est1        &       %est2        &       %est3        &       %est4        \\[-0.15cm]
Crimea S. To $\times$ Post-August 2014&      -2.065$^{**}$ &      -2.760$^{***}$&      -0.737$^{***}$&      -0.854        \\[-0.15cm]
                    &     (1.003)        &     (0.906)        &     (0.264)        &     (0.519)        \\[-0.15cm]\addlinespace[0.15cm] 
Crimea R. From $\times$ Post-August 2014&      -2.436$^{**}$ &      -0.840$^{***}$&      -0.377        &      -0.873$^{***}$\\[-0.15cm]
                    &     (0.918)        &     (0.175)        &     (0.313)        &     (0.306)        \\[-0.15cm]\addlinespace[0.15cm] 
Not Crimea S. To $\times$ Post-August 2014&      -1.779$^{*}$  &      -7.814$^{***}$&      -1.215$^{**}$ &      -1.217$^{**}$ \\[-0.15cm]
                    &     (1.020)        &     (0.584)        &     (0.471)        &     (0.564)        \\[-0.15cm]\addlinespace[0.15cm] 
Not Crimea R. From $\times$ Post-August 2014&      -1.839$^{***}$&      -0.938$^{*}$  &      -1.078$^{***}$&      -1.047$^{***}$\\[-0.15cm]
                    &     (0.484)        &     (0.522)        &     (0.283)        &     (0.192)        \\[-0.15cm]\addlinespace[0.15cm] 
Region From, Region To, Time FEs&{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        \\[-0.15cm]\addlinespace[0.15cm] 

R$^2$               &        0.30        &        0.37        &        0.35        &        0.43        \\[-0.15cm]
Observations        &    {97,040}        &    {97,040}        &    {97,040}        &    {97,040}        \\[-0.15cm]
\addlinespace[0.15cm] 


==> Tables/Table_1_Firm_Month_Nov_2021.tex <==
%                    &       %est1        &       %est2        &       %est3        &       %est4        &       %est5        &       %est6        \\[-0.1cm]
Post Crimea $\times$ &      -0.116$^{***}$&      -0.276$^{***}$&      -1.522$^{***}$&      -0.115$^{***}$&      -0.273$^{***}$&      -1.503$^{***}$\\[-0.1cm]
 \textnormal{ } \textnormal{ }  Either Firm Operated from Conflict Area                    &     (0.005)        &     (0.012)        &     (0.064)        &     (0.005)        &     (0.012)        &     (0.064)        \\[0.1cm]
Post Crimea $\times$ &                    &                    &                    &      -0.029$^{***}$&      -0.065$^{***}$&      -0.381$^{***}$\\[-0.1cm]
\textnormal{ } \textnormal{ } Either Firm Traded with Conflict Areas                    &                    &                    &                    &     (0.003)        &     (0.007)        &     (0.038)        \\[0.1cm]
Establishment-Pair FE        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        \\[-0.1cm]
Year-Month FE       &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        \\

Y Mean              &       0.076        &       0.177        &       0.993        &       0.076        &       0.177        &       0.993        \\[-0.1cm]
Y SD                &       0.265        &       0.716        &       3.487        &       0.265        &       0.716        &       3.487        \\[-0.1cm]
R$^2$               &       0.199        &       0.286        &       0.217        &       0.199        &       0.286        &       0.217        \\[-0.1cm]
Observations        &  10,053,408        &  10,053,408        &  10,053,408        &  10,053,408        &  10,053,408        &  10,053,408        \\[-0.1cm]
Province Pairs       &         711        &         711        &         711        &         711        &         711        &         711        \\


==> Tables/Table_1_Firm_Rayon_Month_BH_Nov_2021.tex <==
%                    &       %est1        &       %est2        &       %est3        &       %est4        &       %est5        &       %est6        \\[-0.1cm]
Post Crimea $\times$&      -0.118$^{***}$&      -0.279$^{***}$&      -1.542$^{***}$&      -0.111$^{***}$&      -0.264$^{***}$&      -1.456$^{***}$\\[-0.1cm]
\textnormal{ } \textnormal{ }  Either Partner is in Conflict Area                    &     (0.005)        &     (0.012)        &     (0.062)        &     (0.005)        &     (0.012)        &     (0.062)        \\[0.1cm]
Post Crimea $\times$ &                    &                    &                    &      -0.024$^{***}$&      -0.056$^{***}$&      -0.317$^{***}$\\[-0.1cm]
 \textnormal{ } \textnormal{ } Either Partner Traded with Conflict Areas                    &                    &                    &                    &     (0.002)        &     (0.005)        &     (0.026)        \\[0.1cm]
Post Crimea $\times$&      -0.000$^{***}$&      -0.001$^{***}$&      -0.004$^{***}$&      -0.000$^{***}$&      -0.001$^{***}$&      -0.004$^{***}$\\[-0.1cm]
 \textnormal{ } \textnormal{ }  Number of Buyer's Partners in 2013                 &     (0.000)        &     (0.000)        &     (0.000)        &     (0.000)        &     (0.000)        &     (0.000)        \\[0.1cm]
Post Crimea $\times$&      -0.000$^{***}$&      -0.000$^{***}$&      -0.001$^{***}$&      -0.000$^{***}$&      -0.000$^{**}$ &      -0.001$^{***}$\\[-0.1cm]
 \textnormal{ } \textnormal{ }  Number of Supplier's Partners in 2013                 &     (0.000)        &     (0.000)        &     (0.000)        &     (0.000)        &     (0.000)        &     (0.000)        \\[0.1cm]
Establishment-Pair FE        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        \\[-0.1cm]
Year-Month FE       &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        \\

Y Mean              &       0.076        &       0.177        &       0.993        &       0.076        &       0.177        &       0.993        \\[-0.1cm]
Y SD                &       0.265        &       0.716        &       3.487        &       0.265        &       0.716        &       3.487        \\[-0.1cm]
R$^2$               &       0.200        &       0.286        &       0.217        &       0.200        &       0.286        &       0.218        \\[-0.1cm]
Observations        &  10,053,408        &  10,053,408        &  10,053,408        &  10,053,408        &  10,053,408        &  10,053,408        \\[-0.1cm]
Province Pairs       &         711        &         711        &         711        &         711        &         711        &         711        \\

==> Tables/Table_1_Firm_Rayon_Month_Nov_2021.tex <==
%                    &       %est1        &       %est2        &       %est3        &       %est4        &       %est5        &       %est6        \\[-0.1cm]
Post Crimea $\times$&      -0.116$^{***}$&      -0.276$^{***}$&      -1.522$^{***}$&      -0.108$^{***}$&      -0.258$^{***}$&      -1.416$^{***}$\\[-0.1cm]
\textnormal{ } \textnormal{ }  Either Partner is in Conflict Area                  &     (0.005)        &     (0.012)        &     (0.064)        &     (0.005)        &     (0.012)        &     (0.064)        \\[0.1cm]
Post Crimea $\times$&                    &                    &                    &      -0.032$^{***}$&      -0.071$^{***}$&      -0.418$^{***}$\\[-0.1cm]
\textnormal{ } \textnormal{ } Either Partner Traded with Conflict Areas      &                    &                    &                    &     (0.002)        &     (0.005)        &     (0.028)        \\[0.1cm]
Establishment-Pair FE        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        \\[-0.1cm]
Year-Month FE       &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        \\

Y Mean              &       0.076        &       0.177        &       0.993        &       0.076        &       0.177        &       0.993        \\[-0.1cm]
Y SD                &       0.265        &       0.716        &       3.487        &       0.265        &       0.716        &       3.487        \\[-0.1cm]
R$^2$               &       0.199        &       0.286        &       0.217        &       0.200        &       0.286        &       0.217        \\[-0.1cm]
Observations        &  10,053,408        &  10,053,408        &  10,053,408        &  10,053,408        &  10,053,408        &  10,053,408        \\[-0.1cm]
Province Pairs       &         711        &         711        &         711        &         711        &         711        &         711        \\


==> Tables/Table_2_Firm_Rayon_Month_UD_Nov_2021.tex <==
%                    &       %est1        &       %est2        &       %est3        &       %est4        &       %est5        &       %est6        \\[-0.1cm]
Post Crimea $\times$&      -0.095$^{***}$&      -0.238$^{***}$&      -1.256$^{***}$&      -0.082$^{***}$&      -0.211$^{***}$&      -1.087$^{***}$\\[-0.1cm]
\textnormal{ } \textnormal{ } Supplier is in Conflict Area                   &     (0.005)        &     (0.013)        &     (0.068)        &     (0.005)        &     (0.013)        &     (0.065)        \\[0.1cm]
Post Crimea $\times$&      -0.145$^{***}$&      -0.329$^{***}$&      -1.888$^{***}$&      -0.129$^{***}$&      -0.295$^{***}$&      -1.681$^{***}$\\[-0.1cm]
\textnormal{ } \textnormal{ } Buyer is in Conflict Area                   &     (0.006)        &     (0.018)        &     (0.086)        &     (0.007)        &     (0.018)        &     (0.089)        \\[0.1cm]
Post Crimea $\times$ &                    &                    &                    &      -0.012$^{***}$&      -0.029$^{***}$&      -0.162$^{***}$\\[-0.1cm]
\textnormal{ } \textnormal{ } Either Partner Had Supplier in Conflict Area                   &                    &                    &                    &     (0.002)        &     (0.005)        &     (0.024)        \\[0.1cm]
Post Crimea $\times$ &                    &                    &                    &      -0.029$^{***}$&      -0.058$^{***}$&      -0.370$^{***}$\\[-0.1cm]
\textnormal{ } \textnormal{ } Either Partner Had Buyer in Conflict Area                   &                    &                    &                    &     (0.003)        &     (0.006)        &     (0.034)        \\[0.1cm]
Establishment-Pair FE        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        \\[-0.1cm]
Year-Month FE       &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        \\

Y Mean              &       0.076        &       0.177        &       0.993        &       0.076        &       0.177        &       0.993        \\[-0.1cm]
Y SD                &       0.265        &       0.716        &       3.487        &       0.265        &       0.716        &       3.487        \\[-0.1cm]
R$^2$               &       0.199        &       0.286        &       0.217        &       0.200        &       0.286        &       0.218        \\[-0.1cm]
Observations        &  10,053,408        &  10,053,408        &  10,053,408        &  10,053,408        &  10,053,408        &  10,053,408        \\[-0.1cm]
Province Pairs       &         711        &         711        &         711        &         711        &         711        &         711        \\


==> Tables/Table_3_Donbas_Crimea.tex <==
%                    &       %est1        &       %est2        &       %est3        &       %est4        &       %est5        &       %est6        \\[-0.1cm]
Post Crimea $\times$  &      -0.194$^{***}$&      -0.462$^{***}$&      -2.557$^{***}$&      -0.203$^{***}$&      -0.482$^{***}$&      -2.679$^{***}$\\[-0.1cm]
\textnormal{ } \textnormal{ } Either Partner is in Crimea      &     (0.008)        &     (0.019)        &     (0.100)        &     (0.008)        &     (0.019)        &     (0.101)        \\[0.1cm]
Post Escalation in Donbas $\times$ &      -0.101$^{***}$&      -0.240$^{***}$&      -1.319$^{***}$&      -0.105$^{***}$&      -0.248$^{***}$&      -1.367$^{***}$\\[-0.1cm]
\textnormal{ } \textnormal{ } Either Partner is in Donbas   &     (0.004)        &     (0.011)        &     (0.050)        &     (0.004)        &     (0.011)        &     (0.054)        \\[0.1cm]
Post Crimea $\times$ &                    &                    &                    &      -0.025$^{***}$&      -0.053$^{***}$&      -0.321$^{***}$\\[-0.1cm]
\textnormal{ } \textnormal{ }  Either Partner Traded with Crimea                  &                    &                    &                    &     (0.002)        &     (0.006)        &     (0.030)        \\[0.1cm]
Post Escalation in Donbas $\times$ &                    &                    &                    &      -0.013$^{***}$&      -0.027$^{***}$&      -0.164$^{***}$\\[-0.1cm]
\textnormal{ } \textnormal{ }   Either Partner Traded with Donbas                  &                    &                    &                    &     (0.002)        &     (0.005)        &     (0.025)        \\[0.1cm]
Firm-Pair FE        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        \\[-0.1cm]
Year-Month FE       &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        &{\checkmark}        \\

Y Mean              &       0.076        &       0.177        &       0.993        &       0.076        &       0.177        &       0.993        \\[-0.1cm]
Y SD                &       0.265        &       0.716        &       3.487        &       0.265        &       0.716        &       3.487        \\[-0.1cm]
R$^2$               &       0.199        &       0.286        &       0.217        &       0.200        &       0.286        &       0.218        \\[-0.1cm]
Observations        &  10,053,408        &  10,053,408        &  10,053,408        &  10,053,408        &  10,053,408        &  10,053,408        \\[-0.1cm]
Province Pairs       &         711        &         711        &         711        &         711        &         711        &         711        \\

